A Survey of Word Reordering in Statistical Machine Translation: Computational Models and Language Phenomena

Word reordering is one of the most difficult aspects of statistical machine translation (SMT), and an important factor of its quality and efficiency. Despite the vast amount of research published to date, the interest of the community in this problem has not decreased, and no single method appears to be strongly dominant across language pairs. Instead, the choice of the optimal approach for a new translation task still seems to be mostly driven by empirical trials. To orientate the reader in this vast and complex research area, we present a comprehensive survey of word reordering viewed as a statistical modeling challenge and as a natural language phenomenon. The survey describes in detail how word reordering is modeled within different string-based and tree-based SMT frameworks and as a stand-alone task, including systematic overviews of the literature in advanced reordering modeling. We then question why some approaches are more successful than others in different language pairs. We argue that, besides measuring the amount of reordering, it is important to understand which kinds of reordering occur in a given language pair. To this end, we conduct a qualitative analysis of word reordering phenomena in a diverse sample of language pairs, based on a large collection of linguistic knowledge. Empirical results in the SMT literature are shown to support the hypothesis that a few linguistic facts can be very useful to anticipate the reordering characteristics of a language pair and to select the SMT framework that best suits them.

==> part-appendices.tex <==
\appendixsection{Reordering constraints TODO}
\label{app:reoconstraints}

 \TOCHECK{TODO}

\noindent To avoid decoding dead-ends, the distortion limit has to be coupled with another constraint (gap constraint)
which ensures that the left-most uncovered input position~($\ell$) will still be reachable after translating the next source phrase.
Formally, to translate a new source interval $J_i$, the gap between $J_i$ and $\ell$ must not exceed the DL:
%
\begin{equation}\label{eq:gap-constraint}
 \left| \ell - \textrm{end}(J_{i}) -1 \right| \ \leq \textrm{DL}
\end{equation}

%%% 
\gap \TOCHECK{TODO}

\begin{itemize} \setlength{\itemsep}{.5mm}\setlength{\parskip}{.5mm} 
\item \textbf{MS (max skip)}: 
at each decoding step, translate one of the first \textit{k} uncovered source positions. In other terms, the translation of a limited number of words (at most \textit{k}) may be postponed indefinitely. 
\item \textbf{IS (inverted skip)}: at each decoding step, check how many source words after the first uncovered position \textit{j} have been translated. If they are less than $k{-}1$, translate any uncovered word, otherwise translate \textit{j}.
This means that the translation of at most $k{-}1$ source words can be anticipated at any point, while the rest of the sentence is covered monotonically.
\end{itemize}
%
The growth of the permutation search space for a sentence of 10 words, with respect to the threshold \textit{k} of the MS, IS and DL constraints is reported in Table \ref{tab:nb_perm}.%
\footnote{For a formal definition and complexity analysis of the DL and IBM constraints, we refer the reader to \namecite{Lopez:09}.} 
We notice that the space defined by DL is considerably smaller than the one defined by IBM constraints, as long as \textit{k} is small compared to the sentence length.
However, both types of constraint grow exponentially with \textit{k}.
The default configuration of the open-source PSMT toolkit Moses \cite{Koehn:07}
includes a DL of 6 words and this is widely accepted as a good baseline setting for many language pairs.

\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\centering  \small
\begin{tabular}{l |r r r r r r r r r} 
\multicolumn{1}{c}{} & \multicolumn{9}{c}{Number of permutations (in thousands)}\\
\cline{1-10}
\ Threshold ($k$): 	& \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{7} & \multicolumn{1}{c}{8} & \multicolumn{1}{c}{9} &10$+$ \\
\hline
\ MS or IS	& 0.5 &	13   & 98 & 375   & 933 & 1729 & 2581 & 3266 & 3629 \\ 
\ DL 	& 0.2 & \ 3  & 24 & 128 & 476 & 1246 & 2333 & 3266 & 3629 \\ 
\hline
\end{tabular}
\caption{\label{tab:nb_perm} 
Number of permutations allowed for a 10-word sentence 
by the maximum skip (MS), inverted skip (IS) and distortion limit (DL) constraints,
while varying the respective thresholds ($k$). The total number of permutations is 10!=3,628,800.}
\end{table}

An enhancement to the IBM constraints was proposed by \namecite{Tillmann:03} 
to specifically address the reordering of verbs between German and English, in a word-based SMT system.
This paradigm allows to set different thresholds for the anticipation and for the postponement of some input words.
A reordering state is added to the decoder to ensure that any reordering pattern (either \textit{skip} or \textit{move}) is completed before initiating a new one. Both reordering patterns are strictly defined and, aside from them, decoding proceeds monotonically.
For the German-English translation direction, 
\namecite{Tillmann:03} manually set their thresholds so that one word may be skipped for at most 4 positions, and up to 2 words may be moved left by at most 10 positions. In this way, a non-contiguous verb chunk in German may be correctly reordered into a contiguous verb chunk in English.
Note, however, that these constraints do not take into account the actual position of the verbs in the input sentence.

%%% 

\COMMENT{
%We have already presented in equation~\eqref{eq:phr-disto} the \textbf{distortion cost} function, which is commonly employed as a basic reordering model by modern PSMT systems, such as Moses.
%
A weakness of this function is that it penalizes long jumps only when they are performed,
rather than accumulating their cost gradually.
As a result, hypotheses with gaps (\ie uncovered input positions) can proliferate and cause the pruning of more monotonic hypotheses that could lead to  overall better translations.%
%
To solve this problem, \namecite{Moore:07} proposed an improved version of the distortion cost function
which consists in ``incorporating an estimate of the distortion penalty yet to be incurred into the estimated score for the
portion of the source sentence remaining to be translated'' (\textbf{early distortion cost}).%
\footnote{A similar idea had been proposed by \namecite{Och:04} for the alignment template SMT approach, under the name of min-jumps.}
This function has the same value as the standard one over a complete translation hypothesis, 
provided that the jump from the last translated word to the end of the sentence is taken into account.
As a difference, though, it anticipates the gradual accumulation of the total distortion cost,
making hypotheses with the same number of covered words more comparable with one another.
%
For instance, in Figure~\ref{fig:running-example-phr},
standard distortion becomes 1 when we skip the first source phrase $J_3$ 
but does not increase while we cover $J_1$ and $J_2$.
Only when we jump back and forth to cover $J_3$ and 
continue, the cost finally increases by +6 and +5 leading to a total of 12.
%
%On the contrary, early distortion cost always includes the minimal cost that will be incurred to cover all current gaps and return to the right-most covered position. 
On the contrary, early distortion is already 6 after the first step: that is, 1 for skipping $J_3$ plus 5 for the minimal future cost.
The second step is monotonic, but the minimal future cost is incremented by 6. 
When we finally jump back and forth to translate $J_3$ and continue, no additional cost is paid, leading to the same total of 12.
%Early distortion cost is computed by an algorithm that keeps track of the uncovered input positions and is available in Moses as a decoding option.
}

%%%%%%%%%%%%%%%%%%%%%%%%%
\appendixsection{Example of KRS computation}
\label{app:krs}

 \TOCHECK{TODO}


%%% EXAMPLE

\begin{figure}[h]
\centering
\includegraphics[width=.7\textwidth]{fig/align2permutation.pdf}
\caption{\label{fig:KRS} {Example of KRS computation showing how word alignments are converted to permutations.}}
\end{figure}

Figure~\ref{fig:KRS} illustrates an example of KRS computation.
A source sentence of 7 words (in the center) is aligned to 
a reference translation of 8 words and to an MT output of 6.
The two word alignment sets are converted to permutations ($\pi$ and $\sigma$) according to the following rules:
(i)   multiple source words aligned to the same target word are considered to be in monotonic order,
(ii)  non-aligned source words are assumed to immediately follow the previous source word, and 
(iii) if a source word is aligned to non-adjacent words in the target, only the first alignment is retained.
Thus, for example, the link \textsc{s2-t5} is ignored, while \textsc{s7} is inserted right after \textsc{s6} in permutation $\sigma$.
The discordant pairs between $\pi$ and $\sigma$ are \textsc{(s1,s2),(s1,s3),(s1,s4),(s5,s6),(s5,s7)}, hence:
\begin{gather}
\nonumber
K(\pi,\sigma) = \frac{5}{\frac{1}{2}7(7-1)} = 0.2381 \quad  \textrm{,}  \quad BP(\pi,\sigma)=\exp \left(1-\frac{8}{6}\right) =0.7165 \\
\nonumber
KRS = (1-\sqrt{0.2381}) \cdot BP = 0.3669
\end{gather}
%
\noindent
In the example of Table~\ref{tab:Birch}, 
hypothesis (a) would obtain a much higher KRS than (b): that is 0.8509 versus 0.2546.



